Too Vivid to Be Real? Benchmarking and Calibrating Generative Color Fidelity

Recent advances in text-to-image (T2I) generation have greatly improved visual quality, yet producing images that appear visually authentic to real-world photography remains challenging. This is partly due to biases in existing evaluation paradigms: human ratings and preference-trained metrics often favor visually vivid images with exaggerated saturation and contrast, which make generations often too vivid to be real even when prompted for realistic-style images. To address this issue, we present Color Fidelity Dataset (CFD) and Color Fidelity Metric (CFM) for objective evaluation of color fidelity in realistic-style generations. CFD contains over 1.3M real and synthetic images with ordered levels of color realism, while CFM employs a multimodal encoder to learn perceptual color fidelity. In addition, we propose a training-free Color Fidelity Refinement (CFR) that adaptively modulates spatial-temporal guidance scale in generation, thereby enhancing color authenticity. Together, CFD supports CFM for assessment, whose learned attention further guides CFR to refine T2I fidelity, forming a progressive framework for assessing and improving color fidelity in realistic-style T2I generation. The dataset and code are available at https://github.com/ZhengyaoFang/CFM.

==> tab/ab_loss.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation on CFS: Softrank vs. pairwise.} 
The softrank loss achieves higher accuracy and human correlation by providing differentiable listwise supervision.}
\small
\setlength{\tabcolsep}{4.2pt}
\scalebox{0.8}{
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{\textbf{Loss}} & \multicolumn{2}{c}{\textbf{CFD-Test Acc. (\%)}} & \multicolumn{2}{c}{\textbf{CFD-Human Corr.}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& \textbf{SynPairs} & \textbf{Real\&Syn} & \textbf{Spearman $\uparrow$} & \textbf{Kendall} $\uparrow$ \\
\midrule
Pairwise & 76.2 & 74.8 & 78.3 & 66.1 \\
Softrank (ours) & \textbf{83.6} & \textbf{80.1} & \textbf{84.9} & \textbf{71.4} \\
\bottomrule
\end{tabular}}
\label{tab:ablation_cfs_loss}
\end{table}

==> tab/ab_modality.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation on CFS: Text-aware vs. visual-only.} 
Textual conditioning significantly enhances color-realism estimation, especially when color appearance is context-dependent.}
\small
\setlength{\tabcolsep}{4.2pt}
\scalebox{0.8}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{CFD-Test Acc. (\%)}} & \multicolumn{2}{c}{\textbf{CFD-Human Corr.}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& \textbf{SynPairs} & \textbf{Real\&Syn} & \textbf{Spearman $\uparrow$} & \textbf{Kendall $\uparrow$} \\
\midrule
Visual-only & 77.1 & 74.3 & 78.9 & 67.0 \\
Text-aware (ours) & \textbf{83.6} & \textbf{80.1} & \textbf{84.9} & \textbf{71.4} \\
\bottomrule
\end{tabular}}

\label{tab:ablation_cfs_text}
\end{table}

==> tab/category.tex <==
\begin{table*}[!t]
\centering
\small

\scalebox{0.75}{
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{l|cccccccccccccccccccccccccc}
\toprule
\textbf{Models} & \textbf{All} && \textbf{Characters} && \textbf{Arts} && \textbf{Design} && \textbf{Architecture} && \textbf{Animals} && \textbf{Natural Scenery} && \textbf{Transportation} && \textbf{Products} && \textbf{Plants} && \textbf{Food} && \textbf{Science} && \textbf{Others} \\
\midrule              
    Kolors \cite{kolors} & && && && && && && && && \\
    Flux-dev~\cite{flux2024} & && && && && && && && && \\
    Playground-v2.5~\cite{playground} & && && && && && && && && \\
    Infinity~\cite{han2024infinity} & && && && && && && && && \\
    CogView4~\cite{cogview3} & && && && && && && && && \\
    PixArt-$\Sigma$~\cite{chen2024pixart} & && && && && && && && && \\
    Gemini 2.0 Flash ~\footnotemark & && && && && && && && && \\
    Stable Diffusion XL~\cite{podell2023sdxl} & && && && && && && && && \\
    Hunyuan~\cite{hunyuandit} & && && && && && && && && \\
    Stable Diffusion 3~\cite{sd3} & && && && && && && && && \\
    Stable Diffusion v2.0~\cite{stable_diffusion} & && && && && && && && && \\
    Qwen Image~\cite{stable_diffusion} & && && && && && && && && \\
\bottomrule
\end{tabular}
}}

\caption{\label{tab:bench_mark_category}\textbf{Ours Benchmark of popular image generation models.} We generate images for each participating model using its recommended inference settings or official API. The best and second-best results are highlighted in \textbf{bold} and \underline{underlined}, respectively. }

\end{table*}

